Off-Policy Multi-Agent Decomposed Policy Gradients

Multi-agent policy gradient (MAPG) methods recently witness vigorous progress. However, there is a significant performance discrepancy between MAPG methods and state-of-the-art multi-agent value-based approaches. In this paper, we investigate causes that hinder the performance of MAPG algorithms and present a multi-agent decomposed policy gradient method (DOP). This method introduces the idea of value function decomposition into the multi-agent actor-critic framework. Based on this idea, DOP supports efficient off-policy learning and addresses the issue of centralized-decentralized mismatch and credit assignment in both discrete and continuous action spaces. We formally show that DOP critics have sufficient representational capability to guarantee convergence. In addition, empirical evaluations on the StarCraft II micromanagement benchmark and multi-agent particle environments demonstrate that DOP significantly outperforms both state-of-the-art value-based and policy-based multi-agent reinforcement learning algorithms. Demonstrative videos are available at https://sites.google.com/view/dop-mapg/.

==> 9-ImpactAck.tex <==
\section*{Broader Impact}
Multi-agent reinforcement learning could be applied to a wide range of applications. However, there is still a gap between state-of-the-art approaches and real-world applications, partly due to instability and sample efficiency. Our DOP method presented in this paper bridges this gap, both theoretically and empirically showing stronger stability and better sample efficiency than existing methods and thus improving the applicability to real-world problems.

Apart from essential advances related to the method itself, multi-agent systems whose development is based on or made use of our approach may contribute to a broad range of uses, including unmanned aerial vehicles control, robot team navigation, control of mobile sensor networks, traffic light control and many more. Each of these applications may have a large range of societal implications. For instance, the use of unmanned aerial vehicles in place of manual control could bring benefits such as cost savings and removing automatic tasks, but could also result in safety problems because of the black-box nature of deep learning.  

In addition to the impacts of the strengths and weaknesses of the technology itself, we also emphasize that depending on who uses this scientific advance and where to apply it, such as criminals for malicious damages or government departments for public services, this technology may be socially harmful or beneficial. 

In general, we see opportunities for applying DOP to beneficial purposes, as well as risks associated with it. To amplify benefits and mitigate risks, we encourage (i) research towards understanding the impacts of using DOP in realistic scenarios; (ii) regulations to confine the usage of related techniques.

